Parameter Efficient Fine Tuning for Multi-scanner PET to PET Reconstruction

Reducing scan time in Positron Emission Tomography (PET) imaging while maintaining high-quality images is crucial for minimizing patient discomfort and radiation exposure. Due to the limited size of datasets and distribution discrepancy across scanners in medical imaging, fine-tuning in a parameter-efficient and effective manner is on the rise. Motivated by the potential of Parameter-Efficient Fine-Tuning (PEFT), we aim to address these issues by effectively leveraging PEFT to improve limited data and GPU resource issues in multi-scanner setups. In this paper, we introduce PETITE, Parameter-Efficient Fine-Tuning for MultI-scanner PET to PET REconstruction that uses fewer than 1% of the parameters. To the best of our knowledge, this study is the first to systematically explore the efficacy of diverse PEFT techniques in medical imaging reconstruction tasks via prevalent encoder-decoder-type deep models. This investigation, in particular, brings intriguing insights into PETITE as we show further improvements by treating encoder and decoder separately and mixing different PEFT methods, namely, Mix-PEFT. Using multi-scanner PET datasets comprised of five different scanners, we extensively test the cross-scanner PET scan time reduction performances (i.e., a model pre-trained on one scanner is fine-tuned on a different scanner) of 21 feasible Mix-PEFT combinations to derive optimal PETITE. We show that training with less than 1% parameters using PETITE performs on par with full fine-tuning (i.e., 100% parameter)

==> Table/gpu.tex <==
%%%%%%%%%%%%%%%%%%%%%%%train,time, gpu memory %%%%%%%%%%%%
\begin{table}[h]
\centering
\caption{In this table, the first row shows the average training time of the methods, and the second raw lists the average GPU memory allocated usage of the methods.}\label{my-label}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cl|ccccccccl}
\toprule
\multicolumn{2}{c|}{Method} & Full-FT & LN   & BitFit   & LoRA   & Adapters & SSF & VPT & Ours \\ 
\midrule
\multicolumn{1}{c|}{3D CVT-GAN} & Train time (sec)  & 430  & 365 & 360 & 368 & 357 & 361 & 378 &      \\
\multicolumn{1}{c|}{}& GPU memory (MB) & & 8,963 & 7,899 & 8,100 & 7,835 & 7,035 & 7,999 & 8,066 &      \\ 
\midrule
\multicolumn{1}{c|}{UNETR} & Train time (sec)  & 481  & 417 & 433 & 415 & 453 & 468 & 424 &      \\
\multicolumn{1}{c|}{}& GPU memory (MB)  & 14,341 & 10,217 & 10,218 & 10,237 & 10,258 & 10,733 & 10,622 &      \\ 
\bottomrule
\end{tabular}%
}
\end{table}

==> sec/ack.tex <==
\subsubsection{\ackname} 
This work was supported in part by the IITP 2020-0-01361 (AI Graduate School Program at Yonsei University), NRF RS-2023-00262002, and NRF RS-2023-00219019 funded by Korean Government (MSIT).

\subsubsection{Disclosure of Interests.} The authors have no competing interests.
